Reinforcement Learning of CPG-regulated Locomotion Controller for a Soft Snake Robot

Intelligent control of soft robots is challenging due to the nonlinear and difficult-to-model dynamics. One promising model-free approach for soft robot control is reinforcement learning (RL). However, model-free RL methods tend to be computationally expensive and data-inefficient and may not yield natural and smooth locomotion patterns for soft robots. In this work, we develop a bio-inspired design of a learning-based goal-tracking controller for a soft snake robot. The controller is composed of two modules: An RL module for learning goal-tracking behaviors given the unmodeled and stochastic dynamics of the robot, and a central pattern generator (CPG) with the Matsuoka oscillators for generating stable and diverse locomotion patterns. We theoretically investigate the maneuverability of Matsuoka CPG's oscillation bias, frequency, and amplitude for steering control, velocity control, and sim-to-real adaptation of the soft snake robot. Based on this analysis, we proposed a composition of RL and CPG modules such that the RL module regulates the tonic inputs to the CPG system given state feedback from the robot, and the output of the CPG module is then transformed into pressure inputs to pneumatic actuators of the soft snake robot. This design allows the RL agent to naturally learn to entrain the desired locomotion patterns determined by the CPG maneuverability. We validated the optimality and robustness of the control design in both simulation and real experiments, and performed extensive comparisons with state-of-art RL methods to demonstrate the benefit of our bio-inspired control design.

==> defs.tex <==
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% based on defs.tex by S. Boyd
% modified by Jie Fu
\newif\ifuseboldmathops
\newif\ifuseittextabbrevs
\useboldmathopstrue   % comment out to use mathbb
%\useittextabbrevstrue % comment out to use non-italic text abbrevs like e.g.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% text abbrevs
\ifuseittextabbrevs
	\newcommand{\cf}{{\it cf.}}
	\newcommand{\eg}{{\it e.g.}}
	\newcommand{\ie}{{\it i.e.}}
	\newcommand{\etc}{{\it etc.}}
	\newcommand{\etal}{{et~al.}}
\else
	\newcommand{\cf}{cf.}
	\newcommand{\eg}{e.g.}
	\newcommand{\ie}{i.e.}
	\newcommand{\etc}{etc.}
	\newcommand{\etal}{et~al.}
\fi

% standard math sets
\ifuseboldmathops
	%\newcommand{\reals}{{\mbox{\bf R}}}
	\newcommand{\reals}{\mathbf{R}}
	\newcommand{\integers}{\mathbf{Z}}
	\newcommand{\complex}{\mathbf{C}}
	\newcommand{\symm}{\mathbf{S}}  % symmetric matrices
\else
	\newcommand{\reals}{\mathbb{R}}
	\newcommand{\integers}{\mathbb{Z}}
	\newcommand{\complex}{\mathbb{C}}
	\newcommand{\symm}{\mathbb{S}}  % symmetric matrices
\fi

% control theory sets
\ifuseboldmathops
	\newcommand{\HH}{\mathbf{H}}
	\newcommand{\LL}{\mathbf{L}}
\else
	\newcommand{\HH}{\mathbb{H}}
	\newcommand{\LL}{\mathbb{L}}
\fi

% probability operators
\ifuseboldmathops
	\newcommand{\Expect}{\mathop{\bf E{}}\nolimits}
	\newcommand{\Prob}{\mathop{\bf P{}}\nolimits}
\else
	\newcommand{\Expect}{\mathop{\mathbb{E}{}}\nolimits}
	\newcommand{\Prob}{\mathop{\mathbb{P}{}}\nolimits}
\fi

% convex operators
\ifuseboldmathops
	\renewcommand{\Re}{\mathop{\bf Re}}
	\renewcommand{\Im}{\mathop{\bf Im}}
	
	\newcommand{\prox}{\mathop{\bf prox}} % proximal operator
	\newcommand{\dom}{\mathop{\bf dom}}   % domain
	\newcommand{\aff}{\mathop{\bf aff}}   % affine hull
	\newcommand{\cl}{\mathop{\bf cl}}     % closure
	\newcommand{\intr}{\mathop{\bf int}}  % interior
	\newcommand{\Co}{\mathop{\bf Co}}     % convex hull
	\newcommand{\relint}{\mathop{\bf rel int}} % relative interior
	\newcommand{\bd}{\mathop{\bf bd}}     % boundary
	
	\newcommand{\Tr}{\mathop{\bf Tr}}
	\newcommand{\diag}{\mathop{\bf diag}}
\else
	\renewcommand{\Re}{\mathop{\mathrm{Re}}}
	\renewcommand{\Im}{\mathop{\mathrm{Im}}}
	
	\newcommand{\prox}{\mathop{\mathrm{prox}}} % proximal operator
	\newcommand{\dom}{\mathop{\mathrm{dom}}}   % domain
	\newcommand{\aff}{\mathop{\mathrm{aff}}}   % affine hull
	\newcommand{\cl}{\mathop{\mathrm{cl}}}     % closure
	\newcommand{\intr}{\mathop{\mathrm{int}}}  % interior
	\newcommand{\Co}{\mathop{\mathrm{Co}}}     % convex hull
	\newcommand{\relint}{\mathop{\mathrm{rel int}}} % relative interior
	\newcommand{\bd}{\mathop{\mathrm{bd}}}     % boundary
	
	\newcommand{\Tr}{\mathop{\mathrm{Tr}}}     % trace
	\newcommand{\diag}{\mathop{\mathrm{diag}}} % diagonal matrix
\fi

% useful non-bold operators
\newcommand{\eqbydef}{\mathrel{\stackrel{\Delta}{=}}}
\newcommand{\eqbyset}{\mathrel{\stackrel{\mathrm{set}}{=}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}

% lin alg stuff
\newcommand{\Span}{\mathop{\mathrm{span}}}
\newcommand{\Range}{\mathop{\mathrm{range}}}
\newcommand{\Null}{\mathop{\mathrm{null}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}

\newcommand{\ones}{\mathbf 1}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{{\lambda_{\rm min}}}
\newcommand{\sigmamax}{{\sigma_{\rm max}}}
\newcommand{\sigmamin}{{\sigma_{\rm min}}}

% linear temporal logic 
% from Baier, Katoen
\newcommand{\truev}{\mathsf{true}}

\newcommand{\falsev}{\mathsf{false}}
\newcommand{\Always}{\Box \, }
\newcommand{\Eventually}{\Diamond \, }
\newcommand{\Next}{\bigcirc \, }
\newcommand{\until}{\mbox{$\, {\sf U}\,$}}
\newcommand{\R}{\mbox{$\, {\sf R}\,$}}
\newcommand{\Unless}{\mbox{$\, {\sf W}\,$}}
\newcommand{\Model}{{\cal K}}


% \newcommand{\Eventually}{\mbox{$\tilde{{\sf F}} \, $}}
% \newcommand{\Untils}{\mbox{$\, \tilde{{\sf U}}\,$}}
% \newcommand{\Alwaysp}{\mbox{${\sf G}^{{-}1} \, $}}
% \newcommand{\Everp}{\mbox{${\sf F}^{{-}1} \, $}}
% \newcommand{\Nextp}{\mbox{${\sf X}^{{-}1} \, $}}


\newcommand{\G}{\Always}
\newcommand{\U}{\Until}
\newcommand{\WU}{\mbox{$\, {\sf W}\,$}}
\newcommand{\Release}{\mbox{$\, {\sf R}\,$}}
\newcommand{\X}{\Next}
%\newcommand{\V}{\mbox{$\, \overline{{\sf U}} \,$}}
\newcommand{\Lagrange}{\mathcal{L}}

%\newcommand{\Always}{\Box \, }
 %\newcommand{\Eventually}{\Diamond \, }
% \newcommand{\Next}{\bigcirc \, }
\newcommand{\sink}{\mathsf{sink} }

%\newcommand{\Next}{\kern0.5ex\vcenter{\hbox{$\scriptstyle\bigcirc$}}\kern0.5ex}
\newcommand{\BoolTrue}{\mbox{\sf true}}
\newcommand{\BoolFalse}{\mbox{\sf false}}
\newcommand{\agg}{\mathcal{A}}
\newcommand{\normal}[1]{\mathcal{N}\left(#1\right)}


\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\grid}[1]{\left[#1\right]}

\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\card}[1]{\mathsf{card}(#1)}

\newcommand{\stateof}[1]{\llbracket#1\rrbracket}

\newcommand{\dist}[1]{\Delta(#1)}
\newcommand{\prob}{\mbox{Prob}}
\newcommand{\update}{\mathsf{update}}

\newcommand{\supp}{\mbox{Supp}}


\newcommand{\labelcost}{\mbox{goal}}
\newcommand{\bigO}{\mathbb{O}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calAP}{\mathcal{AP}}

\newcommand{\fac}{\mathsf{fac}}

\newcommand{\calD}{\mathcal{D}}



\newcommand{\init}{\mathsf{Init}}
\newcommand{\final}{\mathsf{Final}}
\newcommand{\suff}{\mathsf{Suff}}
\newcommand{\last}{\mathsf{Last}}
\newcommand{\semi}{\mathsf{semi}}
\newcommand{\occ}{\mathsf{Occ}}



\newcommand{\guard}{\mathsf{Guard}}
\newcommand{\task}{\mathcal{T}}

\newcommand{\val}{\mathcal{V}}
\newcommand{\prog}{\mathsf{Prog}}



\newcommand{\avoid}{\mathfrak{O}}
\newcommand{\cost}{\mathcal{C}}
\newcommand{\softmax}{\mbox{softmax}}
\newcommand{\softmin}{\mbox{softmin}}

\newcommand{\softidx}{\mbox{softidx}}
\newcommand{\indicator}{\mathbf{1}}

\renewcommand{\vec}[1]{\mathbf{#1}}

\newcommand{\inside}[1]{\llbracket
{#1} \rrbracket
}

\newcommand{\idx}{\mathbf{\eta}}

\newcommand{\nat}{\mathbb{Z}}

\newcommand{\weight}{\mathbf{w}}
\newcommand{\prodInit}{\hat{\mu}} 
\newcommand{\prodP}{\hat{P}} 
\newcommand{\option}{\mathsf{O}} 

% \newcommand{\path}{\mathsf{Path}} 
\newcommand{\win}{\mathsf{Win}} 

% acronym

\acrodef{mdp}[MDP]{Markov Decision Process}
\acrodef{pomdp}[POMDP]{Partially Observable Markov Decision Process}

%%% define the theorem environment

\theoremstyle{definition}
 \newtheorem{definition}{Definition}
 \newtheorem{example}{Example}
\newtheorem{problem}{Problem}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}



\newcommand{\goal}{\mathfrak{g}}

\newcommand{\goals}{\mathsf{G}}
\newcommand{\reach}{\mbox{Reach}}
\newcommand{\caught}{\mbox{Caught}}
\newcommand{\unsafe}{\mbox{Unsafe}}
\newcommand{\hgame}{\mathcal{HG}}


\newcommand{\alg}{\mathsf{ALG}}
%% new operators for game solution
\newcommand{\pre}{\mathsf{Pre}}
\newcommand{\apre}{\mathsf{Apre}}

\newcommand{\vS}{\mathsf{S}}

\newcommand{\vA}{\mathsf{A}}
\newcommand{\vP}{\mathsf{P}}

% symbol for automaton
\newcommand{\calA}{\mathcal{A}}
% symbol for the game
\newcommand{\game}{\mathcal{G}}



\newcommand{\vs}{\mathsf{s}}
\newcommand{\va}{\mathsf{a}}
\newcommand{\vtheta}{\vartheta}

\newcommand{\know}{\vS^{(k)}}

\newcommand{\knows}{\mathcal{K}}

%%% define acronym
\acrodef{smdp}[Semi-MDP]{Semi-Markov decision process}
\acrodef{rl}[RL]{reinforcement learning}
\acrodef{mcts}[MCTS]{Monte Carlo tree search}
\acrodef{uct}[UCT]{Upper Confidence Bound 1 applied to trees}
\acrodef{scltl}[scLTL]{syntactically co-safe LTL}
\acrodef{ssp}[SSP]{Stochastic Shortest Path}
\acrodef{p2sg}[SG(2)]{Two-player Stochastic Game}
\acrodef{dof}[DOF]{degree of freedom}
\acrodef{cpg}[CPG]{Central Pattern Generator}
\acrodef{nn}[NN]{Neural Network}
\acrodef{snn}[SNN]{Spiking Neural Net}
\acrodef{rstdp}[R-STDP]{Reward-Modulated Spike-Timing-Dependent Plasticity}
\acrodef{gp}[GP]{Genetic Programming}
\acrodef{ppoc}[PPOC]{Proximal Policy Optimization Option-Critics}
\acrodef{dr}[DR]{Domain Randomization}
\acrodef{bibo}[BIBO]{Bounded-input, Bounded-Output}

\acrodefplural{dof}[DOFs]{degrees of freedom}
\acrodefplural{cpg}[CPGs]{Central Pattern Generators}

% introduce belief reach-unsafe states in belief mdp
\newcommand{\reachBeliefMDP}{\bar{\mathcal{F}}} % in math environment.
\newcommand{\unsafeBeliefMDP}{\bar{\mathcal{O}}}
